Commissioning of the 2.6 m tall two-phase xenon time projection chamber of Xenoscope

Xenoscope is a demonstrator for a next-generation xenon-based observatory for astroparticle physics, as proposed by the XLZD (XENON-LUX-ZEPLIN-DARWIN) collaboration. It houses a 2.6 m tall, two-phase xenon time projection chamber (TPC), in a cryostat filled with $\sim$ 360 kg of liquid xenon. The main goals of the facility are to demonstrate electron drift in liquid xenon over this distance, to measure the electron cloud transversal and longitudinal diffusion, as well as the optical properties of the medium. In this work, we describe in detail the construction and commissioning of the TPC and report on the observation of light and charge signals with cosmic muons.

==> preamble.tex <==
\usepackage{jinstpub} % for details on the use of the package, please see the JINST-author-manual
\usepackage{lineno}
\usepackage{siunitx}
\usepackage{lipsum}
\usepackage{subcaption}
\usepackage{upgreek}
\usepackage{graphicx}
\usepackage{isotope}
\usepackage{todonotes}
\usepackage{orcidlink}
\usepackage[section]{placeins} % prevent figures from appearing in previous (sub-)sections

\newcommand{\ca}{{\sim}}
\newcommand{\Autoref}[1]{%
	\begingroup%
	\def\chapterautorefname{Chapter}%
	\def\sectionautorefname{Section}%
	\def\subsectionautorefname{Subsection}%
	\autoref{#1}%
	\endgroup%
}

\newlength{\twosubht}
\newsavebox{\twosubbox}

\newcommand{\tbt}{\qtyproduct[product-units = power]{12 x 12}{\mm}}
\newcommand{\sbs}{\qtyproduct[product-units = power]{6 x 6}{\mm}}
\newcommand{\tfbtf}{\qtyproduct[product-units = power]{24 x 24}{\mm}}


%%%% For latexdiff

%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF UNDERLINE PREAMBLE %DIF PREAMBLE
\RequirePackage[normalem]{ulem} %DIF PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
\providecommand{\DIFadd}[1]{{\protect\color{blue}\uwave{#1}}} %DIF PREAMBLE
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}                      %DIF PREAMBLE
%DIF SAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddbegin}{} %DIF PREAMBLE
\providecommand{\DIFaddend}{} %DIF PREAMBLE
\providecommand{\DIFdelbegin}{} %DIF PREAMBLE
\providecommand{\DIFdelend}{} %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}} %DIF PREAMBLE
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}} %DIF PREAMBLE
\providecommand{\DIFaddbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFaddendFL}{} %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFdelendFL}{} %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF
